Small perturbation of a disordered harmonic chain by a noise and an anharmonic potential

We study the thermal properties of a pinned disordered harmonic chain weakly perturbed by a noise and an anharmonic potential. The noise is controlled by a parameter $\lambda \rightarrow 0$, and the anharmonicity by a parameter $\lambda' \le \lambda$. Let $\kappa$ be the conductivity of the chain, defined through the Green-Kubo formula. Under suitable hypotheses, we show that $\kappa = \mathcal O (\lambda)$ and, in the absence of anharmonic potential, that $\kappa \sim \lambda$. This is in sharp contrast with the ordered chain for which $\kappa \sim 1/\lambda$, and so shows the persitence of localization effects for a non-integrable dynamics.

==> Macros.tex <==


% Titres des chapitres (inspir� de  : http://www.grappa.univ-lille3.fr/FAQ-LaTeX/6.17.html, question "Comment modifier les ent�tes de chapitre ?")
\makeatletter
% Titres des chapitres num�rot�s
\def\@makechapterhead#1{%
  \vspace*{50\p@}%
  {\parindent \z@ \centering \normalfont
    \interlinepenalty\@M
    \ifnum \c@secnumdepth >\m@ne
        \Huge \bfseries \thechapter \hspace{0.05cm}  --  
	 \fi
	 \Huge\bfseries #1 \par\nobreak
    \vskip 40\p@
  }}
% Titres des chapitres non num�rot�
\def\@makeschapterhead#1{%
  \vspace*{50\p@}%
  {\parindent \z@ \centering \normalfont
    \interlinepenalty\@M
    \Huge \bfseries  #1\par\nobreak
    \vskip 40\p@
  }}
\makeatother


% Th�or�mes, Propositions, D�finitions ...
\newtheorem{Theorem}{Theorem}
\newtheorem{Proposition}{Proposition}
\newtheorem{Corollary}{Corollary}
\newtheorem{Lemma}{Lemma}
\newtheorem{Definition}{Definition}


% Remark, Proof, Notation... 
% no enumeration
\newcommand{\Proof}{\noindent\emph{Proof.\hspace{0.15cm}}}
\newcommand{\ProofOf}[1]{\noindent\emph{Proof {#1}.\hspace{0.15cm}}}
\newcommand{\Remark}{\noindent\textbf{Remark.\hspace{0.15cm}}}
\newcommand{\Remarks}{\noindent\textbf{Remarks.\hspace{0.15cm}}}
\newcommand{\Convention}{\noindent\emph{Convention.\hspace{0.15cm}}}
\newcommand{\Conventions}{\noindent\emph{Conventions.\hspace{0.15cm}}}
\newcommand{\Notation}{\noindent\emph{Notation.\hspace{0.15cm}}}
\newcommand{\Notations}{\noindent\emph{Notations.\hspace{0.15cm}}}


%\newcounter{CompteurRemark}
%\newcommand{\Remark}
%{
%\refstepcounter{CompteurRemark}
%\noindent\textbf{Remark \theCompteurRemark .\hspace{0.15cm}}
%}


% Espaces de fonctions
\newcommand{\Lp}{\mathrm{L}}
\newcommand{\Cont}{\mathrm{C}}
\newcommand{\BV}{\mathrm{BV}}


% Ensembles
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\T}{\mathbb{T}}


% Normes et valeurs absolues
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\Norm}[1]{\big\lVert #1 \big\rVert}


% Quelques lettres droites
\newcommand{\dd}{\mathrm{d}}
\newcommand{\id}{\mathrm{i}}
\newcommand{\ed}{\mathrm{e}}


% Mesures
\newcommand{\Leb}{m_\mathrm{L}}
\newcommand{\Mean}{\mathsf{E}}
\newcommand{\Proba}{\mathsf{P}}
\newcommand{\Gaussian}{\mathcal{N}}


% Correction de la fermeture de guillemets 
\newcommand{\fgEspace}{\fg \hspace{0.018cm}}


% Autres
\newcommand{\argument}{\, \cdot \,}  
\newcommand{\multiplication}{\, . \,}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\nparticules}{\mathsf n}

